Towards Intelligent Traffic Signaling in Dhaka City Based on Vehicle Detection and Congestion Optimization

The vehicular density in urbanizing cities of developing countries such as Dhaka, Bangladesh result in a lot of traffic congestion, causing poor on-road experiences. Traffic signaling is a key component in effective traffic management for such situations, but the advancements in intelligent traffic signaling have been exclusive to developed countries with structured traffic. The non-lane-based, heterogeneous traffic of Dhaka City requires a contextual approach. This study focuses on the development of an intelligent traffic signaling system feasible in the context of developing countries such as Bangladesh. We propose a pipeline leveraging Real Time Streaming Protocol (RTSP) feeds, a low resources system Raspberry Pi 4B processing, and a state of the art YOLO-based object detection model trained on the Non-lane-based and Heterogeneous Traffic (NHT-1071) dataset to detect and classify heterogeneous traffic. A multi-objective optimization algorithm, NSGA-II, then generates optimized signal timings, minimizing waiting time while maximizing vehicle throughput. We test our implementation in a five-road intersection at Palashi, Dhaka, demonstrating the potential to significantly improve traffic management in similar situations. The developed testbed paves the way for more contextual and effective Intelligent Traffic Signaling (ITS) solutions for developing areas with complicated traffic dynamics such as Dhaka City.

==> tables/model-selection/cpu-env.tex <==
\begin{table}[h]
\caption{Experimental setup for Windows CPU.}
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Attributes} & \textbf{Version/Model}          \\ \hline
Environment         & PC                              \\ \hline
OS                  & Windows 10                      \\ \hline
Python              & 3.9.5                           \\ \hline
Ultralytics         & 8.2.38                          \\ \hline
pytorch             & 2.1.2+cpu                       \\ \hline
GPU                 & -                               \\ \hline
CPU                 & Intel Core(TM) i5-8300H 2.30GHz \\ \hline
\end{tabular}
\label{tab:epu-env}
\end{table}


==> tables/model-selection/gpu-env.tex <==
\begin{table}[h]%
\centering
\caption{Experimental setup for GPU evaluation.}
\begin{tabular}{|c|c|}
\hline
\textbf{Attribute} & \textbf{Value} \\ \hline
Environment & Kaggle \\ \hline
OS & Linux \\ \hline
Python & 3.10.13 \\ \hline
Ultralytics & 8.2.38 \\ \hline
pytorch & 2.1.2 \\ \hline
GPU & Tesla P100-PCIE-16GB, 16276MiB \\ \hline
CUDA & 12.2 \\ \hline
\end{tabular}
\label{tab:model-selection-gpu-env}
\end{table}

==> tables/model-selection/pi-epu-env.tex <==
\begin{table}[h]
\caption{Experimental setup for Windows CPU.}
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Attributes} & \textbf{Version/Model} \\ \hline
Environment         & Raspberry PI 4B        \\ \hline
OS                  & arch64 Linux           \\ \hline
Python              & 3.11.2                 \\ \hline
Ultralytics         & 8.2.38                 \\ \hline
pytorch             & 2.3.1+cpu              \\ \hline
GPU                 & -                      \\ \hline
CPU                 & Cortex-A72             \\ \hline
\end{tabular}
\label{tab:pi-cpu-env}
\end{table}

==> tables/on-road-testing/phase-2-on-road-metric.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Maximum waiting vehicles in a link and average waiting vehicles per link during Phase 2 of on-road testing. The time slots are separated by 1 minute.}
\vspace{-0.25cm}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{|r|rr|rr|}
\hline
\multicolumn{1}{|c|}{\textbf{}}                                                    & \multicolumn{2}{c|}{\textbf{Traffic Police Signaling}}                                                                                                                                                                             & \multicolumn{2}{c|}{\textbf{Proposed System Signaling}}                                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Time\\ slot\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Maximum\\ Waiting\\ Vehicles\\ (in a link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average\\ Waiting\\ Vehicles\\ (per link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Maximum\\ Waiting\\ Vehicles\\ (in a link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average\\ Waiting\\ Vehicles\\ (per link)\end{tabular}}} \\ \hline
1                                                                                  & \multicolumn{1}{r|}{10}                                                                                          & 5.8                                                                                                             & \multicolumn{1}{r|}{8}                                                                                           & 5.4                                                                                                             \\ \hline
2                                                                                  & \multicolumn{1}{r|}{15}                                                                                          & 7.6                                                                                                             & \multicolumn{1}{r|}{20}                                                                                          & 9.6                                                                                                             \\ \hline
3                                                                                  & \multicolumn{1}{r|}{16}                                                                                          & 8.8                                                                                                             & \multicolumn{1}{r|}{17}                                                                                          & 12.2                                                                                                            \\ \hline
4                                                                                  & \multicolumn{1}{r|}{12}                                                                                          & 7.2                                                                                                             & \multicolumn{1}{r|}{18}                                                                                          & 11.2                                                                                                            \\ \hline
5                                                                                  & \multicolumn{1}{r|}{14}                                                                                          & 9                                                                                                               & \multicolumn{1}{r|}{18}                                                                                          & 10.8                                                                                                            \\ \hline
\end{tabular}%
}
\label{tab:phase-2-on-road-metric}
\vspace{-0.65cm}
\end{table}

==> tables/on-road-testing/phase-3-on-road-metric.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Maximum waiting vehicles in a link and average waiting vehicles per link during Phase 3 of on-road testing. The time slots are separated by 30 seconds.}
\vspace{-0.25cm}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|r|rr|rr|}
\hline
\multicolumn{1}{|c|}{\textbf{}}                                                    & \multicolumn{2}{c|}{\textbf{Traffic Police Signaling}}                                                                                                                                                                             & \multicolumn{2}{c|}{\textbf{Proposed System Signaling}}                                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Time\\ slot\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Maximum\\ Waiting\\ Vehicles\\ (in a link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average\\ Waiting\\ Vehicles\\ (per link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Maximum\\ Waiting\\ Vehicles\\ (in a link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average\\ Waiting\\ Vehicles\\ (per link)\end{tabular}}} \\ \hline
1                                                                                  & \multicolumn{1}{r|}{8}                                                                                           & 6.6                                                                                                             & \multicolumn{1}{r|}{4}                                                                                           & 4.2                                                                                                             \\ \hline
2                                                                                  & \multicolumn{1}{r|}{14}                                                                                          & 9.8                                                                                                             & \multicolumn{1}{r|}{16}                                                                                          & 9.4                                                                                                             \\ \hline
3                                                                                  & \multicolumn{1}{r|}{15}                                                                                          & 8.6                                                                                                             & \multicolumn{1}{r|}{18}                                                                                          & 11.2                                                                                                            \\ \hline
4                                                                                  & \multicolumn{1}{r|}{16}                                                                                          & 8.2                                                                                                             & \multicolumn{1}{r|}{15}                                                                                          & 11                                                                                                              \\ \hline
5                                                                                  & \multicolumn{1}{r|}{13}                                                                                          & 8                                                                                                               & \multicolumn{1}{r|}{15}                                                                                          & 9.4                                                                                                             \\ \hline
6                                                                                  & \multicolumn{1}{r|}{12}                                                                                          & 7.4                                                                                                             & \multicolumn{1}{r|}{16}                                                                                          & 10                                                                                                              \\ \hline
7                                                                                  & \multicolumn{1}{r|}{18}                                                                                          & 9.2                                                                                                             & \multicolumn{1}{r|}{18}                                                                                          & 11.4                                                                                                            \\ \hline
8                                                                                  & \multicolumn{1}{r|}{18}                                                                                          & 9.6                                                                                                             & \multicolumn{1}{r|}{21}                                                                                          & 11.6                                                                                                            \\ \hline
9                                                                                  & \multicolumn{1}{r|}{15}                                                                                          & 7.4                                                                                                             & \multicolumn{1}{r|}{12}                                                                                          & 8.4                                                                                                             \\ \hline
10                                                                                 & \multicolumn{1}{r|}{13}                                                                                          & 6.8                                                                                                             & \multicolumn{1}{r|}{20}                                                                                          & 13.2                                                                                                            \\ \hline
\end{tabular}%
}
\label{tab:phase-3-on-road-metric}
\vspace{-0.55cm}
\end{table}

==> tables/on-road-testing/phase-4-on-road-metric.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Maximum waiting vehicles in a link and average waiting vehicles per link during Phase 4 of on-road testing. The time slots are separated by 30 seconds.}
\vspace{-0.25cm}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{|r|rr|rr|}
\hline
\multicolumn{1}{|c|}{\textbf{}}                                                    & \multicolumn{2}{c|}{\textbf{Traffic Police Signaling}}                                                                                                                                                                             & \multicolumn{2}{c|}{\textbf{Proposed System Signaling}}                                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Time\\ slot\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Maximum\\ Waiting\\ Vehicles\\ (in a link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average\\ Waiting\\ Vehicles\\ (per link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Maximum\\ Waiting\\ Vehicles\\ (in a link)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Average\\ Waiting\\ Vehicles\\ (per link)\end{tabular}}} \\ \hline
1                                                                                  & \multicolumn{1}{r|}{6}                                                                                           & 5.4                                                                                                             & \multicolumn{1}{r|}{9}                                                                                           & 6.6                                                                                                             \\ \hline
2                                                                                  & \multicolumn{1}{r|}{12}                                                                                          & 8.2                                                                                                             & \multicolumn{1}{r|}{11}                                                                                          & 7.4                                                                                                             \\ \hline
3                                                                                  & \multicolumn{1}{r|}{14}                                                                                          & 9.4                                                                                                             & \multicolumn{1}{r|}{14}                                                                                          & 8.8                                                                                                             \\ \hline
4                                                                                  & \multicolumn{1}{r|}{13}                                                                                          & 8.4                                                                                                             & \multicolumn{1}{r|}{15}                                                                                          & 9                                                                                                               \\ \hline
5                                                                                  & \multicolumn{1}{r|}{15}                                                                                          & 7.8                                                                                                             & \multicolumn{1}{r|}{14}                                                                                          & 8.6                                                                                                             \\ \hline
6                                                                                  & \multicolumn{1}{r|}{13}                                                                                          & 8.6                                                                                                             & \multicolumn{1}{r|}{15}                                                                                          & 8.8                                                                                                             \\ \hline
7                                                                                  & \multicolumn{1}{r|}{15}                                                                                          & 9.4                                                                                                             & \multicolumn{1}{r|}{17}                                                                                          & 10.2                                                                                                            \\ \hline
8                                                                                  & \multicolumn{1}{r|}{19}                                                                                          & 12                                                                                                              & \multicolumn{1}{r|}{19}                                                                                          & 14                                                                                                              \\ \hline
9                                                                                  & \multicolumn{1}{r|}{20}                                                                                          & 11.8                                                                                                            & \multicolumn{1}{r|}{19}                                                                                          & 12.8                                                                                                            \\ \hline
10                                                                                 & \multicolumn{1}{r|}{19}                                                                                          & 12.4                                                                                                            & \multicolumn{1}{r|}{20}                                                                                          & 12.6                                                                                                            \\ \hline
11                                                                                 & \multicolumn{1}{r|}{21}                                                                                          & 13.8                                                                                                            & \multicolumn{1}{r|}{21}                                                                                          & 12.8                                                                                                            \\ \hline
12                                                                                 & \multicolumn{1}{r|}{22}                                                                                          & 12.2                                                                                                            & \multicolumn{1}{r|}{23}                                                                                          & 13.4                                                                                                            \\ \hline
13                                                                                 & \multicolumn{1}{r|}{20}                                                                                          & 11.6                                                                                                            & \multicolumn{1}{r|}{21}                                                                                          & 13                                                                                                              \\ \hline
14                                                                                 & \multicolumn{1}{r|}{21}                                                                                          & 12.4                                                                                                            & \multicolumn{1}{r|}{22}                                                                                          & 14.2                                                                                                            \\ \hline
\end{tabular}%
}
\label{tab:phase-4-on-road-metric}
\end{table}
